Learning to simulate realistic limit order book markets from data as a World Agent

Multi-agent market simulators usually require careful calibration to emulate real markets, which includes the number and the type of agents. Poorly calibrated simulators can lead to misleading conclusions, potentially causing severe loss when employed by investment banks, hedge funds, and traders to study and evaluate trading strategies. In this paper, we propose a world model simulator that accurately emulates a limit order book market -- it requires no agent calibration but rather learns the simulated market behavior directly from historical data. Traditional approaches fail short to learn and calibrate trader population, as historical labeled data with details on each individual trader strategy is not publicly available. Our approach proposes to learn a unique "world" agent from historical data. It is intended to emulate the overall trader population, without the need of making assumptions about individual market agent strategies. We implement our world agent simulator models as a Conditional Generative Adversarial Network (CGAN), as well as a mixture of parametric distributions, and we compare our models against previous work. Qualitatively and quantitatively, we show that the proposed approaches consistently outperform previous work, providing more realism and responsiveness.

==> CGAN - WorldAgent Model paper (submission) (1)/coletta_comparison.tex <==

  \begin{figure}[t]
\centering
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_real.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Real_distribution_TYPE.png}
  \end{subfigure}
  
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_coletta.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Coletta_et_al_TYPE.png}
  \end{subfigure}
  
    \begin{subfigure}{0.43\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_6b.png} 
  \vspace{-0.15in}
  \end{subfigure}
\centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Explicit_model_TYPE.png}
\vspace{-0.15in}
  \end{subfigure} 
  % 
  
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_gan-v2_4.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/CGAN_model_TYPE.png}
  \end{subfigure}
  
  \caption{\small{Real vs Synthetic order distributions (AVXL). Proposed world models generate more realistic markets compared to previous work: they generate all main market actions which leads to more realistic volumes. }}\label{fig:coletta_comparison}
  \vspace{-0.2in}
  \end{figure}

==> CGAN - WorldAgent Model paper (submission) (1)/coletta_qty.tex <==

  \begin{figure}[t]
\centering
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_real.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Real distribution_TYPE.png}
  \end{subfigure}
  
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_gan-v5.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Coletta et al._TYPE.png}
  \end{subfigure}
  
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_real.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/CGAN model_TYPE.png}
  \end{subfigure}
  
    \begin{subfigure}{0.43\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_6b.png} 
  \end{subfigure}
\centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Explicit model_TYPE.png}
  \end{subfigure} 
  % 
  
  \caption{Real vs Synthetic volume distributions (AVXL).}\label{fig:coletta_comparison}
  \end{figure}

==> CGAN - WorldAgent Model paper (submission) (1)/css.tex <==

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010178</concept_id>
       <concept_desc>Computing methodologies~Artificial intelligence</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010178.10010219.10010220</concept_id>
       <concept_desc>Computing methodologies~Multi-agent systems</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010341</concept_id>
       <concept_desc>Computing methodologies~Modeling and simulation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Artificial intelligence}
\ccsdesc[500]{Computing methodologies~Multi-agent systems}
\ccsdesc[500]{Computing methodologies~Modeling and simulation}


==> CGAN - WorldAgent Model paper (submission) (1)/explicit_model.tex <==


 

% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=2.5cm, sibling distance=3cm]
\tikzstyle{level 2}=[level distance=3cm, sibling distance=1.5cm]
\tikzstyle{level 3}=[level distance=3cm, sibling distance=0.5cm]

% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [circle, minimum width=3pt,fill, inner sep=0pt]


\definecolor{unrelated}{RGB}{255,51,76}  % red
\definecolor{related}{RGB}{85,108,45}  %olivegreen
\definecolor{partialrelated}{RGB}{255,127,0}  % orange

% The sloped option gives rotated edge labels. Personally
% I find sloped labels a bit difficult to read. Remove the sloped options
% to get horizontal labels. 
\begin{tikzpicture}[grow=right, sloped]

    \begin{scope}[xshift=-8cm]
\node[bag] { \Large $\mathcal{F}( \textbf{x} \ | \ \textbf{s}_t )$ }
    child {
        node[bag] {\large CANCEL}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth,} \\ \textbf{queue position)} \end{tabular} 
                    }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | CAN, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | CAN, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth,} \\ \textbf{queue position)} \end{tabular} 
                    }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | CAN, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | CAN, s_t}$}
            }
            edge from parent         
            node[above] {\Large \color{red} $P_{CAN | s_t}$}
 }
    child {
        node[bag] {\large REPLACE}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth, new depth,} \\  \textbf{queue position,} \\ \textbf{new quantity)} \end{tabular} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | REP, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | REP, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                 node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth, new depth,} \\  \textbf{queue position,} \\ \textbf{new quantity)} \end{tabular} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | REP, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | REP, s_t}$}
            }
         edge from parent         
            node[above] {\Large \color{red} $P_{REP | s_t}$}
   }
    child {
        node[bag] {\large ADD MO}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \textbf{(quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{red} $\mathcal{F}(\mathbf{x} \ | MO, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | MO, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                node[end, label=right:
                    {\Large \textbf{(quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{red} $\mathcal{F}(\mathbf{x} \ | MO, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | MO, s_t}$}
            }
        edge from parent         
            node[above] {\Large \color{red} $P_{MO | s_t}$}
    }
    child {
        node[bag] {\large ADD LO}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \textbf{(depth, quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | LO, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | LO, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                node[end, label=right:
                    {\Large \textbf{(depth, quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | LO, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | LO, s_t}$}
            }
        edge from parent         
            node[above] {\Large \color{red} $P_{LO | s_t}$}
    };
\end{scope}

\begin{scope}[yshift=-7cm, xshift=-2cm]
\matrix[column sep=1ex]{
& \path (0,0.5em) node[state,scale=0.5,fill=related,label=right:\huge Related to market state]{};
& \path (0,0.5em) node[state,scale=0.5,fill=partialrelated,label=right:\huge {Partially} related to market state]{};\\
& \path (0,0.5em) node[state,scale=0.5,fill=unrelated,label=right:\huge Un-Related to market state]{};\\
};
\end{scope}

\end{tikzpicture}    

==> CGAN - WorldAgent Model paper (submission) (1)/responsiveness.tex <==

  \begin{figure}[t]
\centering
  \begin{subfigure}{0.22\textwidth} 
  \begin{overpic}[width=\textwidth]{img/impact/6b_10.png} %width=\columnwidth]{img/multi_vs_world_agent}
 \put (35,65) {Explicit Model}
\end{overpic}
%  \includegraphics[width=\textwidth]{img/impact/6b_10.png} 
  \end{subfigure}
  \hfill
\centering
    \begin{subfigure}{0.22\textwidth}
\begin{overpic}[width=\textwidth]{img/impact/gan-v2_4_10.png} %width=\columnwidth]{img/multi_vs_world_agent}
 \put (35,65) {CGAN Model}
\end{overpic}
%  \includegraphics[width=\textwidth]{img/impact/gan-v2_4_10.png}
  \end{subfigure} 
  \hfill
  % 
\centering
  \begin{subfigure}{0.22\textwidth} 
  \includegraphics[width=\textwidth]{img/impact/6b_20.png} 
  \end{subfigure}  
  \hfill
    %
  \centering
  \begin{subfigure}{0.22\textwidth}
  \includegraphics[width=\textwidth]{img/impact/gan-v2_4_20.png}
  \end{subfigure}
  \hfill
  % 
\centering
  \begin{subfigure}{0.22\textwidth} 
  \includegraphics[width=\textwidth]{img/impact/6b_50.png} 
  \end{subfigure}  
  \hfill
    %
  \centering
  \begin{subfigure}{0.22\textwidth}
  \includegraphics[width=\textwidth]{img/impact/gan-v2_4_50.png}
  \end{subfigure}
  \caption{\small{POV Agent Experiment: explicit model (left) and CGAN-based model (right) exhibit price impact and mean reversion trend.}}\label{fig:pov_impact}
  \vspace{-0.1in}
  \end{figure}
  

\begin{comment}

\begin{figure}[t]
\centering
  \begin{subfigure}{0.22\textwidth} 
  \includegraphics[width=\textwidth]{img/impact/6b_20_examples.png} 
  \end{subfigure}
  \hfill
\centering
  \begin{subfigure}{0.22\textwidth}
  \includegraphics[width=\textwidth]{img/impact/gan-v2_4_20_examples.png}
  \end{subfigure} 
\caption{Mid-Price impact samples: implicit agent (left) and CGAN-based model (right).}
\label{fig:pov_agent_samples}
\end{figure}
\end{comment}


==> CGAN - WorldAgent Model paper (submission) (1)/return_stylized.tex <==

  \begin{figure}[t]
\centering
  \begin{subfigure}{0.325\linewidth} 
  \includegraphics[width=1\textwidth]{img/return_stly/MinutelyReturns.png} 
  \end{subfigure}
  \hfill
\centering
  \begin{subfigure}{0.325\linewidth}
  \includegraphics[width=1\textwidth]{img/return_stly/Autocorrelation.png}
  \end{subfigure} 
  \hfill
  % 
  \centering
  \begin{subfigure}{0.325\linewidth}
  \includegraphics[width=1\textwidth]{img/return_stly/VolatilityClustering.png}
  \end{subfigure}
  \vspace{-0.1in}
  \caption{\small{Asset returns stylized fact (AVXL): the world models described in the paper produce stylized facts closer to the historical ones when compared to the multi-agent simulation.}}\label{fig:styl_facts}
  \end{figure}
  

==> CGAN - WorldAgent Model paper (submission) (1)/scalability.tex <==

  \begin{figure}[h]
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/AINV_Explicit Model_depth.png} 
  \end{subfigure}
  \hfill
\centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/AINV_CGAN model_depth.png}
  \end{subfigure} 
  \hfill
  % 
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/CNR_Explicit model_del_depth.png} 
  \end{subfigure}  
  \hfill
    %
  \centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/CNR_CGAN model_del_depth.png}
  \end{subfigure}
  \hfill 
  
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/AMZN_Explicit Model_depth.png} 
  \end{subfigure}
  \hfill
\centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/AMZN_CGAN model_depth.png}
  \end{subfigure} 
  \hfill
  % 
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/AMZN_Explicit Model_SIZEorig.png} 
  \end{subfigure}  
  \hfill
    %
  \centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/AMZN_CGAN model_SIZEorig.png}
  \end{subfigure}

  \caption{Model transferability - AINV, CNR, AMZN. }\label{fig:scalability}
  \end{figure}

==> CGAN - WorldAgent Model paper (submission) (1)/training.tex <==

  \begin{figure}[t]
%    \centering
%  \begin{subfigure}{0.19\textwidth} 
%  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_TYPE.png} 
%  \end{subfigure}
 % \hfill
    %
\centering
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_BUY_SELL_FLAG.png} 
  \end{subfigure}
%   \hfill
 \centering
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/Implicit Model_BUY_SELL_FLAG.png} 
  \end{subfigure}
   \hfill
%---------------%
\centering
  \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_depth.png}
  \end{subfigure}
%  \hfill
    \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/Implicit Model_depth.png}
  \end{subfigure}
  \hfill
  %--------------
\centering
  \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_del_depth.png}
  \end{subfigure} 
  %\hfill
  \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/Implicit Model_del_depth.png}
  \end{subfigure} 
  \hfill
  % --------------
\centering
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_SIZEorig.png} 
  \end{subfigure}  
 % \hfill
%
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/Implicit Model_SIZEorig.png} 
  \end{subfigure}  
  \caption{Implicit model synthetic distributions}
 \label{fig:implic_model}
  \caption{CGAN-based model synthetic distributions (Epoch 15)}
 \label{fig:cgan_model}
\end{figure}



==> CGAN - WorldAgent Model paper (submission) (1)/wa_example.tex <==

 \begin{figure}[b]
 \vspace{-0.1in}
\centering
  \begin{subfigure}{0.45\linewidth}
  \includegraphics[width=\linewidth]{img/imbalance.png}
  \caption{Limit order side probability as a function of market imbalance.}
  \vspace{-0.1in}
  \end{subfigure}
  \hfill
  %
%\centering
  \begin{subfigure}{0.45\linewidth}
  \vspace{-1em}
  \includegraphics[width=\linewidth]{img/interarrival_time.png}
  \caption{Order interarrival times (seconds)}
    \vspace{-0.1in}
  \end{subfigure} 
  \caption{Example of world model distributions.}
  \vspace{-0.1in}
  \label{fig:fitting_wa}
 \end{figure}

==> coletta_qty.tex <==

  \begin{figure}[t]
\centering
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_real.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Real distribution_TYPE.png}
  \end{subfigure}
  
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_gan-v5.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Coletta et al._TYPE.png}
  \end{subfigure}
  
\centering
  \begin{subfigure}{0.445\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_real.png} 
  \end{subfigure}  
    %
  \centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/CGAN model_TYPE.png}
  \end{subfigure}
  
    \begin{subfigure}{0.43\linewidth} 
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/qty_6b.png} 
  \end{subfigure}
\centering
  \begin{subfigure}{0.33\linewidth}
  \includegraphics[width=\textwidth]{img/new_vs_old_gan/Explicit model_TYPE.png}
  \end{subfigure} 
  % 
  
  \caption{Real vs Synthetic volume distributions (AVXL).}\label{fig:coletta_comparison}
  \end{figure}

==> css.tex <==

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010178</concept_id>
       <concept_desc>Computing methodologies~Artificial intelligence</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010178.10010219.10010220</concept_id>
       <concept_desc>Computing methodologies~Multi-agent systems</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010341</concept_id>
       <concept_desc>Computing methodologies~Modeling and simulation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computing methodologies~Artificial intelligence}
\ccsdesc[500]{Computing methodologies~Multi-agent systems}
\ccsdesc[500]{Computing methodologies~Modeling and simulation}


==> explicit_model.tex <==


 

% Set the overall layout of the tree
\tikzstyle{level 1}=[level distance=2.5cm, sibling distance=3cm]
\tikzstyle{level 2}=[level distance=3cm, sibling distance=1.5cm]
\tikzstyle{level 3}=[level distance=3cm, sibling distance=0.5cm]

% Define styles for bags and leafs
\tikzstyle{bag} = [text width=4em, text centered]
\tikzstyle{end} = [circle, minimum width=3pt,fill, inner sep=0pt]


\definecolor{unrelated}{RGB}{255,51,76}  % red
\definecolor{related}{RGB}{85,108,45}  %olivegreen
\definecolor{partialrelated}{RGB}{255,127,0}  % orange

% The sloped option gives rotated edge labels. Personally
% I find sloped labels a bit difficult to read. Remove the sloped options
% to get horizontal labels. 
\begin{tikzpicture}[grow=right, sloped]

    \begin{scope}[xshift=-8cm]
\node[bag] { \Large $\mathcal{F}( \textbf{x} \ | \ \textbf{s}_t )$ }
    child {
        node[bag] {\large CANCEL}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth,} \\ \textbf{queue position)} \end{tabular} 
                    }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | CAN, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | CAN, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth,} \\ \textbf{queue position)} \end{tabular} 
                    }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | CAN, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | CAN, s_t}$}
            }
            edge from parent         
            node[above] {\Large \color{red} $P_{CAN | s_t}$}
 }
    child {
        node[bag] {\large REPLACE}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth, new depth,} \\  \textbf{queue position,} \\ \textbf{new quantity)} \end{tabular} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | REP, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | REP, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                 node[end, label=right:
                    {\Large \begin{tabular}{c}  \textbf{(cancel depth, new depth,} \\  \textbf{queue position,} \\ \textbf{new quantity)} \end{tabular} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | REP, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | REP, s_t}$}
            }
         edge from parent         
            node[above] {\Large \color{red} $P_{REP | s_t}$}
   }
    child {
        node[bag] {\large ADD MO}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \textbf{(quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{red} $\mathcal{F}(\mathbf{x} \ | MO, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | MO, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                node[end, label=right:
                    {\Large \textbf{(quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{red} $\mathcal{F}(\mathbf{x} \ | MO, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | MO, s_t}$}
            }
        edge from parent         
            node[above] {\Large \color{red} $P_{MO | s_t}$}
    }
    child {
        node[bag] {\large ADD LO}        
        child {
            node[bag] {\large BUY}        
            child {
                node[end, label=right:
                    {\Large \textbf{(depth, quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | LO, BUY, s_t)$}
            }
               edge from parent         
            node[below] {\Large \color{OliveGreen} $P_{BUY | LO, s_t}$}
            }
        child {
            node[bag] {\large SELL}        
            child {
                node[end, label=right:
                    {\Large \textbf{(depth, quantity)} }] {}
                edge from parent
                node[above]  {\Large \color{orange} $\mathcal{F}(\mathbf{x} \ | LO, SELL, s_t)$}
            }
               edge from parent         
            node[above] {\Large \color{OliveGreen} $P_{SELL | LO, s_t}$}
            }
        edge from parent         
            node[above] {\Large \color{red} $P_{LO | s_t}$}
    };
\end{scope}

\begin{scope}[yshift=-7cm, xshift=-2cm]
\matrix[column sep=1ex]{
& \path (0,0.5em) node[state,scale=0.5,fill=related,label=right:\huge Related to market state]{};
& \path (0,0.5em) node[state,scale=0.5,fill=partialrelated,label=right:\huge {Partially} related to market state]{};\\
& \path (0,0.5em) node[state,scale=0.5,fill=unrelated,label=right:\huge Un-Related to market state]{};\\
};
\end{scope}

\end{tikzpicture}    

==> scalability.tex <==

  \begin{figure}[h]
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/AINV_Explicit Model_depth.png} 
  \end{subfigure}
  \hfill
\centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/AINV_CGAN model_depth.png}
  \end{subfigure} 
  \hfill
  % 
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/CNR_Explicit model_del_depth.png} 
  \end{subfigure}  
  \hfill
    %
  \centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/CNR_CGAN model_del_depth.png}
  \end{subfigure}
  \hfill 
  
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/AMZN_Explicit Model_depth.png} 
  \end{subfigure}
  \hfill
\centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/AMZN_CGAN model_depth.png}
  \end{subfigure} 
  \hfill
  % 
\centering
  \begin{subfigure}{0.11\textwidth} 
  \includegraphics[width=\textwidth]{img/scalability/AMZN_Explicit Model_SIZEorig.png} 
  \end{subfigure}  
  \hfill
    %
  \centering
  \begin{subfigure}{0.11\textwidth}
  \includegraphics[width=\textwidth]{img/scalability/AMZN_CGAN model_SIZEorig.png}
  \end{subfigure}

  \caption{Model transferability - AINV, CNR, AMZN. }\label{fig:scalability}
  \end{figure}

==> training.tex <==

  \begin{figure}[t]
%    \centering
%  \begin{subfigure}{0.19\textwidth} 
%  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_TYPE.png} 
%  \end{subfigure}
 % \hfill
    %
\centering
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_BUY_SELL_FLAG.png} 
  \end{subfigure}
%   \hfill
 \centering
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/Implicit Model_BUY_SELL_FLAG.png} 
  \end{subfigure}
   \hfill
%---------------%
\centering
  \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_depth.png}
  \end{subfigure}
%  \hfill
    \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/Implicit Model_depth.png}
  \end{subfigure}
  \hfill
  %--------------
\centering
  \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_del_depth.png}
  \end{subfigure} 
  %\hfill
  \begin{subfigure}{0.40\linewidth}
  \includegraphics[width=\textwidth]{img/training/Implicit Model_del_depth.png}
  \end{subfigure} 
  \hfill
  % --------------
\centering
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/CGAN-based Model_SIZEorig.png} 
  \end{subfigure}  
 % \hfill
%
  \begin{subfigure}{0.40\linewidth} 
  \includegraphics[width=\textwidth]{img/training/Implicit Model_SIZEorig.png} 
  \end{subfigure}  
  \caption{Implicit model synthetic distributions}
 \label{fig:implic_model}
  \caption{CGAN-based model synthetic distributions (Epoch 15)}
 \label{fig:cgan_model}
\end{figure}



==> wa_example.tex <==

 \begin{figure}[b]
 \vspace{-0.1in}
\centering
  \begin{subfigure}{0.45\linewidth}
  \includegraphics[width=\linewidth]{img/imbalance.png}
  \caption{Limit order side probability as a function of market imbalance.}
  \vspace{-0.1in}
  \end{subfigure}
  \hfill
  %
%\centering
  \begin{subfigure}{0.45\linewidth}
  \vspace{-1em}
  \includegraphics[width=\linewidth]{img/interarrival_time.png}
  \caption{Order interarrival times (seconds)}
    \vspace{-0.1in}
  \end{subfigure} 
  \caption{Example of world model distributions.}
  \vspace{-0.1in}
  \label{fig:fitting_wa}
 \end{figure}
